MIA 2022 Shared Task: Evaluating Cross-lingual Open-Retrieval Question Answering for 16 Diverse Languages

We present the results of the Workshop on Multilingual Information Access (MIA) 2022 Shared Task, evaluating cross-lingual open-retrieval question answering (QA) systems in 16 typologically diverse languages. In this task, we adapted two large-scale cross-lingual open-retrieval QA datasets in 14 typologically diverse languages, and newly annotated open-retrieval QA data in 2 underrepresented languages: Tagalog and Tamil. Four teams submitted their systems. The best system leveraging iteratively mined diverse negative examples and larger pretrained models achieves 32.2 F1, outperforming our baseline by 4.5 points. The second best system uses entity-aware contextualized representations for document retrieval, and achieves significant improvements in Tamil (20.8 F1), whereas most of the other systems yield nearly zero scores.

==> deprecated/custom_old.tex <==
% Use this file for citations not found in the ACL Anthology (contained in "anthology.bib").

@book{Aho:72,
    author  = {Alfred V. Aho and Jeffrey D. Ullman},
    title   = {The Theory of Parsing, Translation and Compiling},
    year    = "1972",
    volume  = "1",
    publisher = {Prentice-Hall},
    address = {Englewood Cliffs, NJ}
}

@book{APA:83,
    author  = {{American Psychological Association}},
    title   = {Publications Manual},
    year    = "1983",
    publisher = {American Psychological Association},
    address = {Washington, DC}
}

@article{Chandra:81,
	author = {Ashok K. Chandra and Dexter C. Kozen and Larry J. Stockmeyer},
	year = "1981",
	title = {Alternation},
	journal = {Journal of the Association for Computing Machinery},
	volume = "28",
	number = "1",
	pages = "114--133",
	doi = "10.1145/322234.322243",
}

@inproceedings{andrew2007scalable,
  title={Scalable training of {L1}-regularized log-linear models},
  author={Andrew, Galen and Gao, Jianfeng},
  booktitle={Proceedings of the 24th International Conference on Machine Learning},
  pages={33--40},
  year={2007},
}

@book{Gusfield:97,
    author  = {Dan Gusfield},
    title   = {Algorithms on Strings, Trees and Sequences},
    year    = "1997",
    publisher = {Cambridge University Press},
    address = {Cambridge, UK}
}

@article{rasooli-tetrault-2015,
    author    = {Mohammad Sadegh Rasooli and Joel R. Tetreault},
    title     = {Yara Parser: {A} Fast and Accurate Dependency Parser},
    journal   = {Computing Research Repository},
    volume    = {arXiv:1503.06733},
    year      = {2015},
    url       = {http://arxiv.org/abs/1503.06733},
    note    = {version 2}
}

@article{Ando2005,
	Acmid = {1194905},
	Author = {Ando, Rie Kubota and Zhang, Tong},
	Issn = {1532-4435},
	Issue_Date = {12/1/2005},
	Journal = {Journal of Machine Learning Research},
	Month = dec,
	Numpages = {37},
	Pages = {1817--1853},
	Publisher = {JMLR.org},
	Title = {A Framework for Learning Predictive Structures from Multiple Tasks and Unlabeled Data},
	Volume = {6},
	Year = {2005}
}

@article{longpre2021mkqa,
  title={MKQA: A Linguistically Diverse Benchmark for Multilingual Open Domain Question Answering},
  author={Longpre, Shayne and Lu, Yi and Daiber, Joachim},
  journal={Transactions of the Association for Computational Linguistics},
  volume={9},
  pages={1389--1406},
  year={2021},
  publisher={MIT Press}
}

@inproceedings{asai2021xor,
  title={XOR QA: Cross-lingual Open-Retrieval Question Answering},
  author={Asai, Akari and Kasai, Jungo and Clark, Jonathan H and Lee, Kenton and Choi, Eunsol and Hajishirzi, Hannaneh},
  booktitle={Proceedings of the 2021 Conference of the North American Chapter of the Association for Computational Linguistics: Human Language Technologies},
  pages={547--564},
  year={2021}
}

@article{kwiatkowski2019natural,
  title={Natural questions: a benchmark for question answering research},
  author={Kwiatkowski, Tom and Palomaki, Jennimaria and Redfield, Olivia and Collins, Michael and Parikh, Ankur and Alberti, Chris and Epstein, Danielle and Polosukhin, Illia and Devlin, Jacob and Lee, Kenton and others},
  journal={Transactions of the Association for Computational Linguistics},
  volume={7},
  pages={453--466},
  year={2019},
  publisher={MIT Press}
}

@inproceedings{
asai2021cora,
title={One Question Answering Model for Many Languages with Cross-lingual Dense Passage Retrieval},
author={Akari Asai and Xinyan Yu and Jungo Kasai and Hannaneh Hajishirzi},
booktitle={NeurIPS},
year={2021}
}

@INPROCEEDINGS{97cross-languageinformation,
    author = {Peter Schäuble and Páraic Sheridan},
    title = {Cross-Language Information Retrieval (CLIR) Track Overview},
    booktitle = {In Proceedings of the Sixth Text Retrieval Conference (TREC-6},
    year = {1997}
}

@inproceedings{10.5555/1813809.1813852,
author = {Forner, Pamela and Pe\~{n}as, Anselmo and Agirre, Eneko and Alegria, I\~{n}aki and For\u{a}scu, Corina and Moreau, Nicolas and Osenova, Petya and Prokopidis, Prokopis and Rocha, Paulo and Sacaleanu, Bogdan and Sutcliffe, Richard and Sang, Erik Tjong Kim},
title = {Overview of the Clef 2008 Multilingual Question Answering Track},
year = {2008},
isbn = {3642044468},
publisher = {Springer-Verlag},
address = {Berlin, Heidelberg},
abstract = {The QA campaign at CLEF 2008 [1], was mainly the same as that proposed last year. The results and the analyses reported by last year's participants suggested that the changes introduced in the previous campaign had led to a drop in systems' performance. So for this year's competition it has been decided to practically replicate last year's exercise. Following last year's experience some QA pairs were grouped in clusters. Every cluster was characterized by a topic (not given to participants). The questions from a cluster contained coreferences between one of them and the others. Moreover, as last year, the systems were given the possibility to search for answers in Wikipedia as document corpus beside the usual newswire collection. In addition to the main task, three additional exercises were offered, namely the Answer Validation Exercise (AVE), the Question Answering on Speech Transcriptions (QAST), which continued last year's successful pilots, together with the new Word Sense Disambiguation for Question Answering (QA-WSD). As general remark, it must be said that the main task still proved to be very challenging for participating systems. As a kind of shallow comparison with last year's results the best overall accuracy dropped significantly from 42% to 19% in the multi-lingual subtasks, but increased a little in the monolingual sub-tasks, going from 54% to 63%.},
booktitle = {Proceedings of the 9th Cross-Language Evaluation Forum Conference on Evaluating Systems for Multilingual and Multimodal Information Access},
pages = {262–295},
numpages = {34},
location = {Aarhus, Denmark},
series = {CLEF'08}
}

@article{roy2022information,
  title={Information asymmetry in Wikipedia across different languages: A statistical analysis},
  author={Roy, Dwaipayan and Bhatia, Sumit and Jain, Prateek},
  journal={Journal of the Association for Information Science and Technology},
  volume={73},
  number={3},
  pages={347--361},
  year={2022},
  publisher={Wiley Online Library}
}


@InProceedings{pmlr-v133-min21a,
  title = 	 {NeurIPS 2020 EfficientQA Competition: Systems, Analyses and Lessons Learned},
  author =       {Min, Sewon and Boyd-Graber, Jordan and Alberti, Chris and Chen, Danqi and Choi, Eunsol and Collins, Michael and Guu, Kelvin and Hajishirzi, Hannaneh and Lee, Kenton and Palomaki, Jennimaria and Raffel, Colin and Roberts, Adam and Kwiatkowski, Tom and Lewis, Patrick and Wu, Yuxiang and K\"uttler, Heinrich and Liu, Linqing and Minervini, Pasquale and Stenetorp, Pontus and Riedel, Sebastian and Yang, Sohee and Seo, Minjoon and Izacard, Gautier and Petroni, Fabio and Hosseini, Lucas and Cao, Nicola De and Grave, Edouard and Yamada, Ikuya and Shimaoka, Sonse and Suzuki, Masatoshi and Miyawaki, Shumpei and Sato, Shun and Takahashi, Ryo and Suzuki, Jun and Fajcik, Martin and Docekal, Martin and Ondrej, Karel and Smrz, Pavel and Cheng, Hao and Shen, Yelong and Liu, Xiaodong and He, Pengcheng and Chen, Weizhu and Gao, Jianfeng and Oguz, Barlas and Chen, Xilun and Karpukhin, Vladimir and Peshterliev, Stan and Okhonko, Dmytro and Schlichtkrull, Michael and Gupta, Sonal and Mehdad, Yashar and Yih, Wen-tau},
  booktitle = 	 {Proceedings of the NeurIPS 2020 Competition and Demonstration Track},
  pages = 	 {86--111},
  year = 	 {2021},
  editor = 	 {Escalante, Hugo Jair and Hofmann, Katja},
  volume = 	 {133},
  series = 	 {Proceedings of Machine Learning Research},
  month = 	 {06--12 Dec},
  publisher =    {PMLR},
  pdf = 	 {http://proceedings.mlr.press/v133/min21a/min21a.pdf},
  url = 	 {https://proceedings.mlr.press/v133/min21a.html},
  abstract = 	 {We review the EfficientQA competition from NeurIPS 2020. The competition focused on open-domain question answering (QA), where systems take natural language questions as input and return natural language answers.  The aim of the competition was to build systems that can predict correct answers while also satisfying strict on-disk memory budgets. These memory budgets were designed to encourage contestants to  explore  the  trade-off between storing retrieval corpora or the parameters of learned models. In this report, we describe the motivation and organization of the competition, review the best submissions, and analyze system predictions to inform a discussion of evaluation for open-domain QA. }
}

@article{lewis2020retrieval,
  title={Retrieval-augmented generation for knowledge-intensive nlp tasks},
  author={Lewis, Patrick and Perez, Ethan and Piktus, Aleksandra and Petroni, Fabio and Karpukhin, Vladimir and Goyal, Naman and K{\"u}ttler, Heinrich and Lewis, Mike and Yih, Wen-tau and Rockt{\"a}schel, Tim and others},
  journal={Advances in Neural Information Processing Systems},
  volume={33},
  pages={9459--9474},
  year={2020}
}

@article{guu2020realm,
  title={Realm: Retrieval-augmented language model pre-training},
  author={Guu, Kelvin and Lee, Kenton and Tung, Zora and Pasupat, Panupong and Chang, Ming-Wei},
  journal={arXiv preprint arXiv:2002.08909},
  year={2020}
}

@inproceedings{khan-etal-2022-watclaimcheck,
    title = "{W}at{C}laim{C}heck: A new Dataset for Claim Entailment and Inference",
    author = "Khan, Kashif  and
      Wang, Ruizhe  and
      Poupart, Pascal",
    booktitle = "Proceedings of the 60th Annual Meeting of the Association for Computational Linguistics (Volume 1: Long Papers)",
    month = may,
    year = "2022",
    address = "Dublin, Ireland",
    publisher = "Association for Computational Linguistics",
    url = "https://aclanthology.org/2022.acl-long.92",
    pages = "1293--1304",
    abstract = "We contribute a new dataset for the task of automated fact checking and an evaluation of state of the art algorithms. The dataset includes claims (from speeches, interviews, social media and news articles), review articles published by professional fact checkers and premise articles used by those professional fact checkers to support their review and verify the veracity of the claims. An important challenge in the use of premise articles is the identification of relevant passages that will help to infer the veracity of a claim. We show that transferring a dense passage retrieval model trained with review articles improves the retrieval quality of passages in premise articles. We report results for the prediction of claim veracity by inference from premise articles.",
}

@inproceedings{
dinan2018wizard,
title={Wizard of Wikipedia: Knowledge-Powered Conversational Agents},
author={Emily Dinan and Stephen Roller and Kurt Shuster and Angela Fan and Michael Auli and Jason Weston},
booktitle={International Conference on Learning Representations},
year={2019},
url={https://openreview.net/forum?id=r1l73iRqKm},
}

@article{ri2021mluke,
  title={mLUKE: The Power of Entity Representations in Multilingual Pretrained Language Models},
  author={Ri, Ryokan and Yamada, Ikuya and Tsuruoka, Yoshimasa},
  journal={arXiv preprint arXiv:2110.08151},
  year={2021}
}

@inproceedings{izacard2021leveraging,
  title={Leveraging Passage Retrieval with Generative Models for Open Domain Question Answering},
  author={Izacard, Gautier and Grave, Edouard},
  booktitle={EACL 2021-16th Conference of the European Chapter of the Association for Computational Linguistics},
  pages={874--880},
  year={2021},
  organization={Association for Computational Linguistics}
}

@article{wang2022sncse,
  title={SNCSE: Contrastive Learning for Unsupervised Sentence Embedding with Soft Negative Samples},
  author={Wang, Hao and Li, Yangguang and Huang, Zhen and Dou, Yong and Kong, Lingpeng and Shao, Jing},
  journal={arXiv preprint arXiv:2201.05979},
  year={2022}
}

@inproceedings{dugan2022feasibility,
  title={A Feasibility Study of Answer-Unaware Question Generation for Education},
  author={Dugan, Liam and Miltsakaki, Eleni and Upadhyay, Shriyash and Ginsberg, Etan and Gonzalez, Hannah and Choi, DaHyeon and Yuan, Chuning and Callison-Burch, Chris},
  booktitle={Findings of the Association for Computational Linguistics: ACL 2022},
  pages={1919--1926},
  year={2022}
}


@inproceedings{blasi-etal-2022-systematic,
    title = "Systematic Inequalities in Language Technology Performance across the World{'}s Languages",
    author = "Blasi, Damian  and
      Anastasopoulos, Antonios  and
      Neubig, Graham",
    booktitle = "Proceedings of the 60th Annual Meeting of the Association for Computational Linguistics (Volume 1: Long Papers)",
    month = may,
    year = "2022",
    address = "Dublin, Ireland",
    publisher = "Association for Computational Linguistics",
    url = "https://aclanthology.org/2022.acl-long.376",
    pages = "5486--5505",
    abstract = "Natural language processing (NLP) systems have become a central technology in communication, education, medicine, artificial intelligence, and many other domains of research and development. While the performance of NLP methods has grown enormously over the last decade, this progress has been restricted to a minuscule subset of the world{'}s $\approx$6,500 languages. We introduce a framework for estimating the global utility of language technologies as revealed in a comprehensive snapshot of recent publications in NLP. Our analyses involve the field at large, but also more in-depth studies on both user-facing technologies (machine translation, language understanding, question answering, text-to-speech synthesis) as well as foundational NLP tasks (dependency parsing, morphological inflection). In the process, we (1) quantify disparities in the current state of NLP research, (2) explore some of its associated societal and academic factors, and (3) produce tailored recommendations for evidence-based policy making aimed at promoting more global and equitable language technologies. Data and code to reproduce the findings discussed in this paper areavailable on GitHub (https://github.com/neubig/globalutility).",
}

@inproceedings{
izacard2021distilling,
title={Distilling Knowledge from Reader to Retriever for Question Answering},
author={Gautier Izacard and Edouard Grave},
booktitle={International Conference on Learning Representations},
year={2021},
url={https://openreview.net/forum?id=NTEz-6wysdb}
}
